Aligned SICs and embedded tight frames in even dimensions

Alignment is a geometric relation between pairs of Weyl-Heisenberg SICs, one in dimension $d$ and another in dimension $d(d-2)$, manifesting a well-founded conjecture about a number-theoretical connection between the SICs. In this paper, we prove that if $d$ is even, the SIC in dimension $d(d-2)$ of an aligned pair can be partitioned into $(d-2)^2$ tight $d^2$-frames of rank $d(d-1)/2$ and, alternatively, into $d^2$ tight $(d-2)^2$-frames of rank $(d-1)(d-2)/2$. The corresponding result for odd $d$ is already known, but the proof for odd $d$ relies on results which are not available for even $d$. We develop methods that allow us to overcome this issue. In addition, we provide a relatively detailed study of parity operators in the Clifford group, emphasizing differences in the theory of parity operators in even and odd dimensions and discussing consequences due to such differences. In a final section, we study implications of alignment for the symmetry of the SIC.

==> settings.tex <==
\usepackage{amsmath,amssymb,amsfonts,amsthm,bbm,bm,color,array} % Use \bm{} for bold math fonts
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage[utf8]{inputenc} % Any characters can be typed directly from the keyboard, eg éçñ
\usepackage[protrusion=true,expansion=true]{microtype}
\usepackage{textcomp} % provide lots of new symbols

%\addtolength{\textwidth}{20pt}
%\addtolength{\hoffset}{-10pt}
\linespread{1.05}


%\usepackage{nomencl} % to create a list of symbols
%\usepackage{fancyhdr} 
%\pagestyle{fancy} 
%\include{modifyfancy}
%hidelinks,pagebackref,
\usepackage[pdftex,bookmarks,colorlinks,breaklinks]{hyperref}  % PDF hyperlinks, with coloured links
\usepackage{xcolor}
\definecolor{dullmagenta}{rgb}{0.4,0,0.4}   % #660066
\definecolor{darkblue}{rgb}{0,0,0.4}
\hypersetup{linkcolor=red,citecolor=blue,filecolor=dullmagenta,urlcolor=darkblue} % coloured links
%\hypersetup{linkcolor=black,citecolor=black,filecolor=black,urlcolor=black} % black links, for printed output

\usepackage[pdftex]{graphicx}

%\usepackage{tikz-cd} 
%\usetikzlibrary{matrix,arrows,decorations.pathmorphing}

\usepackage{pdfsync}



%%% Theorem styles %%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{conv}{Convention}
\newtheorem{notation}{Notation}

\newtheorem{conjecture}{Conjecture}
\newtheorem{assumption}{Assumption}

\newtheorem*{remark*}{Remark}
\newtheorem*{example*}{Example}

==> shorthands.tex <==
% Number rings
\newcommand{\ints}{\mathbb Z}
\newcommand{\reals}{\mathbb R}
\newcommand{\comps}{\mathbb C}
%\renewcommand{\Re}{\operatorname{Re}}
%\renewcommand{\Im}{\operatorname{Im}}

% Spaces
\newcommand{\HH}{\mathcal{H}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\EE}{\mathcal{E}}
%\newcommand{\DD}{\mathcal{D}}
%\newcommand{\PP}{\mathcal{P}}
%\newcommand{\KK}{\mathcal{K}}
\newcommand{\MM}{\mathcal{M}}
%\newcommand{\TT}{\mathcal{T}}
%\newcommand{\WW}{\mathcal{W}}
\renewcommand{\SS}{\mathcal{S}}
%\newcommand{\SSS}{\mathcal{S}^\circ}
%\newcommand{\CC}{\mathcal{C}}
\newcommand{\FF}{\mathcal{F}}
%\newcommand{\Gr}{\operatorname{Gr}}
%\newcommand{\St}{\operatorname{St}}

% Groups and Algebras
\newcommand{\WH}{\mathrm{WH}}
\newcommand{\C}{\mathrm{C}}
%\newcommand{\GL}{\mathrm{GL}}
\newcommand{\SL}{\mathrm{SL}}
%\newcommand{\UU}{\mathrm{U}}
%\newcommand{\SU}{\mathrm{SU}}
%\newcommand{\uu}{\mathfrak{u}}
%\newcommand{\su}{\mathfrak{su}}
%\newcommand{\hh}{\mathfrak{h}}
%\newcommand{\sh}{\mathfrak{sh}}
%\newcommand{\mm}{\mathfrak{m}}
%\newcommand{\Ad}{\operatorname{Ad}}
%\newcommand{\ad}{\operatorname{ad}}
%\newcommand{\SO}{\mathrm{SO}}
%\newcommand{\SL}{\mathrm{SL}}
%\newcommand{\OO}{\mathrm{O}}
%\newcommand{\GG}{\mathrm{G}}
%\renewcommand{\gg}{\mathfrak{g}}

% Operators
\newcommand{\1}{\mathbbm{1}}
%\newcommand{\0}{\mathbf{0}}
%\renewcommand{\P}{\mathbf{P}}
%\renewcommand{\P}{\mathbf{P}}
%\newcommand{\J}{\mathbf{J}}
%\newcommand{\R}{\mathbf{R}}
%\renewcommand{\L}{\mathbf{L}}
%\newcommand{\II}{\mathcal{I}}
%\newcommand{\JJ}{\mathcal{J}}

% Differential operators
%\newcommand{\pa}{\partial}
%\renewcommand{\d}{\operatorname{d}}
%\newcommand{\ddd}{\operatorname{d}}
%\newcommand{\dd}[1]{\frac{\operatorname{d}}{\operatorname{d}\!#1}}
%\newcommand{\ddt}{\frac{\operatorname{d}}{\operatorname{d}\!t}}
%\newcommand{\ddtva}[1]{\frac{\operatorname{d}^2}{\operatorname{d}\!{#1}^2}}

% Measures
%\newcommand{\dt}{\operatorname{d}\!t}
%\newcommand{\ds}{\!\operatorname{d}\!s}
%\newcommand{\dl}{\mathrm{d}\lambda}
%\newcommand{\domega}{\operatorname{d}\!\omega}

% Functors
%\newcommand{\T}{\operatorname{T}\!}
%\newcommand{\V}{\operatorname{V}\!}
%\renewcommand{\H}{\operatorname{H}\!}
%\newcommand{\HB}{\operatorname{H}^{\textsc{B}}}
%\newcommand{\HWY}{\operatorname{H}^{{}_\textsc{WY}}}
%\newcommand{\HRLD}{\operatorname{H}^{\textrm{RLD}}}

% Distance functions
%\newcommand{\dist}{\operatorname{dist}}
%\newcommand{\Dist}{\operatorname{Dist}}
%\newcommand{\distB}{\operatorname{dist}_{\textsc{b}}}
%\newcommand{\distWY}{\operatorname{dist}_{\textsc{wy}}}
%\newcommand{\distTr}[2]{\operatorname{Dist}_{\textit{Tr}}(#1,#2)}
%\newcommand{\distH}[2]{\operatorname{Dist}_{\textit{H}}(#1,#2)}
%\newcommand{\distV}[2]{\operatorname{Dist}_{\textit{V}}(#1,#2)}
%\newcommand{\angleB}[2]{\operatorname{Angle}_{\textit{B}}(#1,#2)}
%\newcommand{\distFS}[2]{\operatorname{dist}_{\textsc{fs}}(#1,#2)}
%\newcommand{\IWY}{\operatorname{I}_{\textsc{wy}}}

% Metrics
%\newcommand{\GHS}{G_{\textsc{hs}}}
%\newcommand{\GB}{G_{\textsc{b}}}
%\newcommand{\GWY}{G_{\textsc{wy}}}
%\newcommand{\GRLD}{G_{\textsc{rld}}}
%\newcommand{\gFS}{g_{\textsc{fs}}}
%\newcommand{\gF}{g_{\textsc{f}}}
%\newcommand{\gB}{g_{\textsc{b}}}
%\newcommand{\gE}{g_{\textsc{e}}}
%\newcommand{\gU}{g_{\textsc{u}}}
%\newcommand{\gWY}{g_{\textsc{wy}}}
%\newcommand{\gKKS}{g_{\textsc{kks}}}
%\newcommand{\gC}{g_{\textsc{c}}}
%\newcommand{\GammaL}{\Gamma^\textrm{L}}
%\newcommand{\GammaS}{\Gamma^\textrm{S}}
%\newcommand{\GammaR}{\Gamma^\textrm{R}}
%\newcommand{\GammaBKM}{\Gamma^\textrm{BKM}}

% Statistical measures
%\newcommand{\E}{\mathbb{E}}
%\newcommand{\var}{\operatorname{var}}
%\newcommand{\dev}{\operatorname{Dev}}
%\newcommand{\cov}{\operatorname{Cov}}

% Connections and curvature
%\newcommand{\A}{\mathcal{A}}
\newcommand{\AB}{\mathcal{A}_{\textsc{b}}}
%\newcommand{\AWY}{\mathcal{A}_{\textsc{wy}}}
%\newcommand{\Ac}{\mathcal{A}_{\textsc{c}}}
\newcommand{\F}{\mathcal{F}}
%\newcommand{\Hol}{\mathfrak{H}}
%\newcommand{\p}{\Pi}
%\newcommand{\geop}{\gamma_{\text{geo}}}

% Symplectic forms
%\newcommand{\OHS}{\Omega_{\textsc{hs}}}
%\newcommand{\oKKS}{\omega_{\textit{kks}}}

% Dirac notation
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\braket}[2]{\langle #1|#2\rangle}
\newcommand{\ketbra}[2]{|#1\rangle\langle #2|}
%\newcommand{\la}{\langle}
%\newcommand{\ra}{\rangle}

% Functionals
%\newcommand{\length}[1]{\operatorname{Length}[#1]}
%\newcommand{\energy}[1]{\operatorname{Energy}[#1]}

% Miscellaneous
\renewcommand{\r}{\mathbf{r}}
%\newcommand{\Ker}{\operatorname{ker}}
%\newcommand{\Ran}{\operatorname{ran}}
\newcommand{\Tr}{\operatorname{tr}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Rk}{\operatorname{rank}}
%\newcommand{\grad}{\operatorname{grad}}
%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\spec}{\operatorname{spec}}
%\newcommand{\linspan}{\operatorname{span}}
%\renewcommand{\th}{\text{th}}
%\newcommand{\st}{\text{st}}
%\newcommand{\texp}{\operatorname{T}\!\exp}
%\newcommand{\obs}[1]{\mathbf{#1}}
%\newcommand{\eps}{\epsilon}
\newcommand{\md}{\text{ mod }}

% Quantum speed limits
%\newcommand{\tMT}{\tau_\textsc{mt}}
%\newcommand{\tF}{\tau_\textsc{f}}
%\newcommand{\tU}{\tau_\textsc{u}}
%\newcommand{\tT}{\tau_\textsc{t}}
%\newcommand{\tM}{\tau_\textsc{m}}
%\newcommand{\tWY}{\tau_\textsc{wy}}

% Phases
%\newcommand{\tglob}{\theta_{\text{glob}}}
%\newcommand{\ttot}{\theta_{\text{tot}}}
%\newcommand{\tdyn}{\theta_{\text{dyn}}}
%\newcommand{\tgeo}{\theta_{\text{geo}}}
%\newcommand{\Geop}{\Phi_{\text{geo}}}

% Spectra
%\newcommand{\bfp}{\boldsymbol{p}}
%\newcommand{\bfP}{\boldsymbol{P}}
%\newcommand{\bfm}{\boldsymbol{m}}
%\newcommand{\bfPi}{\boldsymbol{\Pi}}
%\newcommand{\bfL}{\boldsymbol{\Lambda}}
%\newcommand{\bfl}{\boldsymbol{\lambda}}

% Matrices
\newcommand{\XXX}{\mathbb{X}}
\newcommand{\ZZZ}{\mathbb{Z}}
\newcommand{\FFF}{\mathbb{F}}
\newcommand{\UUU}{\mathbb{U}}
\newcommand{\VVV}{\mathbb{V}}
\newcommand{\WWW}{\mathbb{W}}
\newcommand{\III}{\mathbb{I}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\rk}{\operatorname{Rank}}
%\newcommand{\Q}{\mathcal{Q}}
%\newcommand{\B}{\mathcal{B}}
%\newcommand{\K}{\operatorname{K}}
%\newcommand{\M}{\mathcal{M}}
%\newcommand{\JJ}{\mathfrak{J}}
%\newcommand{\D}{\operatorname{D}}
%\newcommand{\G}{\mathcal{G}}
%\newcommand{\g}{\mathfrak{g}}
%\newcommand{\bfsigma}{\boldsymbol{\sigma}}
%\renewcommand{\phi}{\varphi}
%\newcommand{\II}{\mathfrak{I}}
%\newcommand{\ptexp}{\operatorname{exp_{+}\!}}
%\newcommand{\ntexp}{\operatorname{exp_{--}\!}}
%\newcommand{\geopf}{\zeta_{\text{geo}}}
%\newcommand{\obs}[1]{\hat{#1}}
